On Estimates for Maximal Operators Associated with Tangential Regions

The thesis comprises three chapters. Chapter 1 investigates generalizations of the theorem of Fatou for convolution type integral operators with general approximate identities. It is introduced $\lambda(r)$-convergence, which is a generalization of non-tangential convergence in the unit disc. The connections between general approximate identities and optimal convergence regions for such operators are described in different functional spaces. Chapter 2 studies some generalizations of the theorem of Littlewood, which makes an important complement to the theorem of Fatou, constructing analytic function possessing almost everywhere divergent property along a given tangential curve. The same convolution type integral operators are considered with more general kernels than approximate identities. Two kinds of generalizations of the theorem of Littlewood are obtained, possessing everywhere divergent property. Chapter 3 is devoted to some questions of equivalency of differentiation bases in $\mathbb{R}^n$. The complete equivalence of basis of rare dyadic rectangles and the basis of complete dyadic rectangles in $\mathbb{R}^2$ is investigated. Besides, it is introduced quasi-equivalence between two differentiation bases in $\mathbb{R}^n$ and is considered the set of functions that such bases differentiate.

==> sections/1.4.tex <==
\begin{proof}[Proof of \trm{1.weakpp}]
Without loss of generality we may assume that $f$ is non-negative.
% Furthermore, we may assume that $\TPI_p\ge C_\varphi^p$ and $\lambda(r)\|\varphi_r\|_\infty\varphi_*^{p-1}(r)\ge C_\varphi^p$ for all $r\in(0,1)$. Otherwise, instead of $\lambda(r)$ we would define a new $\bar{\lambda}(r)$ as
% \begin{equation*}
% \bar{\lambda}(r) \deff \frac{\max\left(\TPI_p, C_\varphi^p\right)}{\|\varphi_r\|_\infty\varphi_*^{p-1}(r)} \ge \lambda(r), \quad 0<r<1,
% \end{equation*}
% for which those assumptions would hold. Denote $\mu(r)=\varphi_*(r)/\|\varphi_r\|_\infty$ and notice that
% \begin{equation*}
% \lambda(r) \ge \frac{C_\varphi^p}{\|\varphi_r\|_\infty\varphi_*^{p-1}(r)} \ge \frac{\varphi_*(r)}{\|\varphi_r\|_\infty}=\mu(r), \quad 0<r<1.
% \end{equation*}

Let $x,y\in\ZT,\,0<r<1$ and $|x-y|<\lambda(r)$. We split the integral $\Phi_r(y,f)$ as follows
\md9\label{1.I123}
\Phi_r(y,f)
&= \int_\ZT \varphi_r(t)f(y-t)\,dt\\
&= \int_{|t|\le\mu(r)} \varphi_r(t)f(y-t)\,dt\\
&+ \int_{\mu(r)<|t|<\lambda(r)} \varphi_r(t)f(y-t)\,dt\\
&+ \int_{\lambda(r)\le|t|\le\pi} \varphi_r(t)f(y-t)\,dt = I^1 + I^2 + I^3.
\emd
First of all, from \lem{1.Phi*ineq1} we have
\md1\label{1.I3ineq}
\sup_{\substack{|x-y|<\lambda(r)\\0<r<1}} |I^3| \le 8 C_\varphi\cdot Mf(x).
\emd
Notice that from the condition $\TPI_p(\lambda, \varphi)<\infty$ it follows that
\md0
\lambda(r)\le \TPI_p\cdot\mu(r)\FI^{-p}(r).
\emd
Hence, from \lem{1.lemma-supmulambda} we get
\md1\label{1.I2ineq}
\sup_{\substack{|x-y|<\lambda(r)\\0<r<1}} |I^2| \le \frac{4\TPI_p^{1/p}}{2^{1/p}-1} \left(Mf^p(x)\right)^{1/p}.
\emd
Furthermore, using the definition of $\mu(r)$, for $I_1$ we obtain
\md8
|I^1|
&\le \int_{|t|\le\mu(r)} \varphi^*_r(t)f(y-t)\\
&\le \|\varphi_r\|_\infty \int_{-\mu(r)}^{\mu(r)}f(y-t)\,dt\\
&=  2\mu(r)\|\varphi_r\|_\infty m_f(y,\mu(r)) =  2\FI(r)m_f(y,\mu(r)),
\emd
where
\md0
m_f(y,t) = \frac{1}{2t}\int_{y-t}^{y+t}|f(u)|\,du, \quad y\in\ZT,\,t>0.
\emd
To estimate $I_1$ we split the supremum into two parts as we did in \lem{1.lemma-supmulambda}:
\md9\label{1.I1ineq}
\sup_{\substack{|x-y|\le\mu(r)\le\lambda(r)\\0<r<1}} I^1
&\le \sup_{\substack{|x-y|\le\mu(r)\le\lambda(r)\\0<r<1}} 2\FI(r)m_f(y,\mu(r))\\
&+ \sup_{\substack{\mu(r)<|x-y|<\lambda(r)\\0<r<1}} 2\FI(r)m_f(y,\mu(r))
\emd
Notice that the second supremum is $T_1 f(x)$, which can be estimated due to \lem{1.lemma-TAbound}. To estimate the first one, note that $\mu(r)\le\lambda(r)\le \TPI_p\mu(r)\FI(r)^{-p}$ implies
\md1\label{1.varphi-ineq}
\FI(r)\le\TPI_p^{1/p}.
\emd
On the other hand, from $|x-y|\le\mu(r)$ implies $m_f(y,\mu(r))\le Mf(x)$, which together with \e{1.I1ineq}, \e{1.varphi-ineq} and \lem{1.lemma-TAbound} gives
\md9\label{1.I1ineq-1}
\sup_{\substack{|x-y|\le\mu(r)\le\lambda(r)\\0<r<1}} |I^1| \le 2\TPI_p^{1/p} \left(Mf^p(x)\right)^{1/p}.
\emd
Then, combining \e{1.I3ineq}, \e{1.I2ineq}, \e{1.I1ineq-1} and \e{1.I123}, we get
\md0
\sup_{\substack{|x-y|<\lambda(r)\\0<r<1}} \Phi_r(y,f)
\le \left( 2\TPI_p^{1/p} + \frac{4\TPI_p^{1/p}}{2^{1/p}-1} + 8 C_\varphi\right) \left(Mf^p(x)\right)^{1/p},
\emd
which implies \e{1.Phi*-bound}.

To get weak type inequality for $\Phi^*_\lambda$, note that
\md2
\left|\left\{x\in\ZT \colon \Phi_{\lambda}^*(x,f) > t\right\}\right|
&= \left|\left\{x\in\ZT \colon \left(\Phi_{\lambda}^*(x,f)\right)^p > t^p\right\}\right|\\
&\le \left|\left\{x\in\ZT \colon Mf^p(x) > t^p/C^p\right\}\right|\\
&\le \frac{C_MC^p}{t^p} \|f^p\|_1 = \frac{C_MC^p}{t^p} \|f\|_p^p,
\emd
where $C_M=\|M\|_{L^1\to L^{1,w}}$ is the weak $(1,1)$ norm of the maximal operator $M$.
\end{proof}


\begin{proof}[Proof of \trm{1.fatouLp}]
We show that for any function $f\in L^p(\ZT)$ and for any $t>0$, the set
\md0
E_t = \left\{x\in\ZT\colon \left|\limsup_{\stackrel{r\to 1}{y\in\lambda(r,x)}}\Phi_r(y,f)-f(x)\right|>t\right\}
\emd
has measure zero, which obviously will prove the theorem. First note that from the condition $\PI_p(\lambda,\varphi)<\infty$ it follows that
\md0
\sup_{r_0<r<1} \lambda(r)\|\varphi_r\|_{\infty}\FI(r)^{p-1} < \infty,
\emd
for some $r_0\in(0,1)$, hence from \trm{1.weakpp} we have that $\Phi^*_\lambda$ is of weak type $(p,p)$, where $r$ varies in $(r_0,1)$ instead of $(0,1)$. For a given $\varepsilon>0$ we can fix such $g\in C(\ZT)$ that $\|h\|_p<\varepsilon$, where $h=f-g\in L^p(\ZT)$. From \lem{1.lemma-fatouC} it follows that for any $x\in\ZT$ we have
\md0
\lim_{\stackrel{r\to 1}{y\in\lambda(r,x)}}\Phi_r(y,g) = g(x).
\emd
Therefore
\md9\label{1.Et}
E_t
&= \left\{x\in\ZT\colon \left|\limsup_{\stackrel{r\to 1}{y\in\lambda(r,x)}}\Phi_r(y,h)-h(x)\right|>t\right\}\\
&\subset \left\{x\in\ZT\colon \left|\limsup_{\stackrel{r\to 1}{y\in\lambda(r,x)}}\Phi_r(y,h)\right|>\frac{t}{2}\right\}
\cup \left\{x\in\ZT\colon |h(x)|>\frac{t}{2}\right\}\\
&\subset \left\{x\in\ZT\colon \Phi^*_\lambda(x,h)>\frac{t}{2}\right\} \cup \left\{x\in\ZT\colon |h(x)|>\frac{t}{2}\right\}.
\emd
From the weak type inequality of $\Phi^*_\lambda$ we have
\md0
\left|\left\{x\in\ZT\colon \Phi^*_\lambda(x,h)>\frac{t}{2}\right\}\right| \le \frac{2^p\tilde{C}}{t^p}\|h\|_p^p
\le \frac{2^p\tilde{C}}{t^p}\varepsilon^p,
\emd
and applying Chebyshev\a s inequality we obtain
\md0
\left|\left\{x\in\ZT\colon |h(x)|>\frac{t}{2}\right\}\right| \le \frac{2^p}{t^p}\|h\|_p^p \le \frac{2^p}{t^p}\varepsilon^p.
\emd
Combining these two inequalities with \e{1.Et}, we get
\md0
|E_t| \le \frac{2^p(\tilde{C}+1)}{t^p}\varepsilon^p.
\emd
Since $\varepsilon>0$ is arbitrary, we get $|E_t|=0$.
\end{proof}

\begin{proof}[Proof of \trm{1.fatouLp-example}]
From \e{1.extraCondition-phi} it follows that there exists $r_0\in(0,1)$ such that
\md1\label{1.cvarphi}
\frac{1}{\FI(r)}\int_{-\mu(r)}^{\mu(r)}|\varphi_r(t)|\,dt \ge \frac{c_\varphi}{2}
\emd
for any $r,\,r_0<r<1$. Denote
\md5
n(r) = \left[\frac{4\pi}{\lambda(r)}\right]\in\ZN,\label{1.nr}\\
\Delta_r = \bigcup_{k=0}^{n(r)-1}\left[\frac{2\pi k}{n(r)} - \mu(r), \frac{2\pi k}{n(r)} + \mu(r)\right],\label{1.Deltar}\\
\Lambda(r) = \lambda(r)\|\varphi_r\|_\infty\FI^{p-1}(r),\label{1.Lambdar}
\emd
If $x\in\ZT$ is an arbitrary point and $r_0<r<1$, then
\md0
x\in\left[\frac{2\pi k_0}{n(r)}, \frac{2\pi(k_0+1)}{n(r)}\right)
\emd
for some $k_0\in\{0, 1, \dots, n(r)-1\}$. Consider the function
\md1\label{1.fr-def}
f_r(x) = \frac{\Lambda^{1/p}(r)}{\FI(r)}\ZI_{\Delta_r}(x) \cdot \sgn\varphi_r\left(\frac{2\pi k_0}{n(r)}-x\right).
\emd
Note that
\md9\label{1.fr-Lp}
\|f_r\|_p^p
= \frac{\Lambda(r)}{\FI^p(r)}\cdot |\Delta_r| &= \frac{\Lambda(r)}{\FI^p(r)}\cdot 2\mu(r)n(r)\\
&\le \frac{\lambda(r)\|\varphi_r\|_\infty\FI^{p-1}(r)}{\FI^p(r)}\cdot\frac{2\FI(r)}{\|\varphi_r\|_\infty}\cdot\frac{4\pi}{\lambda(r)} = 8\pi.
\emd
Clearly, taking $\theta = x-2\pi k_0/n(r)$, from \e{1.nr} we obtain
\md1\label{1.theta-bound}
|\theta| < \frac{2\pi}{n(r)} < \lambda(r).
\emd
Using the condition $\PI_p(\lambda, \varphi)=\infty$ and \lem{1.BV-means}, we may fix a sequence $r_k\nearrow 1$ such that
\md3
&\Lambda(r_k) > \left[2^{k+1}C_\varphi\cdot c_\varphi^{-1}\left(8\pi + k +\max_{1\le j<k}\frac{\Lambda^{1/p}(r_j)}{\FI(r_j)}\right)\right]^p,\quad  k=1,2,\ldots ,\label{1.Lambda-bound}\\
&\sup_{\theta\in\ZT}\frac{1}{|\Delta_{r_j}|}\int_{\Delta_{r_j}} \varphi^*_{r_k}(\theta-t)\,dt \le C_\varphi,\quad k=1, 2, \dots, j-1.\label{1.phi-bound-uniform}
\emd
Using \e{1.cvarphi} and \e{1.fr-def}, we get
\md9\label{1.Phir-bound-below}
\Phi_r(x-\theta,f_r)
&= \int_{\ZT} \varphi_r\left(\frac{2\pi k_0}{n(r)}-t\right)f_r(t)\,dt\\
&= \frac{\Lambda^{1/p}(r)}{\FI(r)} \int_{\Delta_r} \left|\varphi_r\left(\frac{2\pi k_0}{n(r)}-t\right)\right|\,dt\\
&\ge \frac{\Lambda^{1/p}(r)}{\FI(r)} \int_{2\pi k_0/n(r)-\mu(r)}^{2\pi k_0/n(r)+\mu(r)} \left|\varphi_r\left(\frac{2\pi k_0}{n(r)}-t\right)\right|\,dt\\
&= \frac{\Lambda^{1/p}(r)}{\FI(r)} \int_{-\mu(r)}^{\mu(r)} \left|\varphi_r(u)\right|du
\ge \frac{c_\varphi}{2} \Lambda^{1/p}(r).
\emd
Define
\md0
f(x)=\sum_{k=1}^\infty 2^{-k}f_{r_k}(x)\in L^p(\ZT).
\emd
We split $\Phi_{r_k}(\theta,f)$ in the following way
\md9\label{1.Phi-split-Lp}
\Phi_{r_k}(\theta,f)
&= \sum_{j=1}^\infty 2^{-j}\Phi_{r_k}(\theta, f_{r_j})\\
&= \sum_{j=1}^{k-1} 2^{-j}\Phi_{r_k}(\theta, f_{r_j}) + 2^{-k}\Phi_{r_k}(\theta, f_{r_k}) + \sum_{j=k+1}^\infty 2^{-j}\Phi_{r_k}(\theta, f_{r_j})\\
&= S^1 + S^2 + S^3.
\emd
From \e{1.theta-bound}, \e{1.Lambda-bound}, and \e{1.Phir-bound-below} it follows that
\md9\label{1.bound-S2-Lp}
\sup_{y\in\lambda(r_k,x)} S^2
&= \sup_{y\in\lambda(r_k,x)} 2^{-k}\Phi_{r_k}(y,f_{r_k})\\
&\ge 2^{-k}\Phi_{r_k}(x-\theta,f_{r_k})\\
&\ge 2^{-k-1}c_\varphi\Lambda^{1/p}(r_k)
\ge C_\varphi \left(8\pi + k +\max_{1\le j<k}\frac{\Lambda^{1/p}(r_j)}{\FI(r_j)}\right).
\emd
Furthermore, using \e{1.fr-def} and propery $\mathit{\Phi3}$, we get
\md9\label{1.bound-S1-Lp}
\sup_{\theta\in\lambda(r_k,x)} |S^1|
&= \sup_{\theta\in\lambda(r_k,x)} \left|\sum_{j=1}^{k-1} 2^{-j}\int_\ZT \varphi_{r_k}(\theta-t)f_{r_j}(t)\,dt\right|\\
&\le \sup_{\theta\in\lambda(r_k,x)} \sum_{j=1}^{k-1} 2^{-j}\frac{\Lambda^{1/p}(r_j)}{\FI(r_j)} \int_{\Delta_{r_j}}|\varphi_{r_k}(\theta-t)|\,dt\\
&\le \sum_{j=1}^{k-1} 2^{-j}\frac{\Lambda^{1/p}(r_j)}{\FI(r_j)} \int_\ZT\varphi^*_{r_k}(u)\,du
\le C_\varphi\cdot\max_{1\le j<k} \frac{\Lambda^{1/p}(r_j)}{\FI(r_j)}.
\emd
Finally, using \e{1.fr-Lp} and \e{1.phi-bound-uniform} we get
\md9\label{1.bound-S3-Lp}
\sup_{\theta\in\lambda(r_k,x)} |S^3|
&= \sup_{\theta\in\lambda(r_k,x)} \left|\sum_{j=k+1}^\infty 2^{-j}\int_\ZT \varphi_{r_k}(\theta-t)f_{r_j}(t)\,dt\right|\\
&\le \sup_{\theta\in\lambda(r_k,x)} \sum_{j=k+1}^\infty 2^{-j}\frac{\Lambda^{1/p}(r_j)}{\FI(r_j)} \int_{\Delta_{r_j}}|\varphi_{r_k}(\theta-t)|\,dt\\
&\le \sum_{j=k+1}^\infty 2^{-j}\frac{\Lambda^{1/p}(r_j)}{\FI(r_j)}|\Delta_{r_j}|\cdot\sup_{\theta\in\ZT}\frac{1}{|\Delta_{r_j}|} \int_{\Delta_{r_j}}\varphi^*_{r_k}(\theta-t)\,dt \le 8\pi\cdot C_\varphi.
\emd
So, from \e{1.bound-S1-Lp}, \e{1.bound-S2-Lp}, \e{1.bound-S3-Lp} and \e{1.Phi-split-Lp} it follows
\md0
\sup_{\theta\in\lambda(r_k,x)} \Phi_{r_k}(\theta,f)
\ge \sup_{\theta\in\lambda(r_k,x)} S^2 - \sup_{\theta\in\lambda(r_k,x)} |S^1| - \sup_{\theta\in\lambda(r_k,x)} |S^3|
\ge C_\varphi\cdot k,
\emd
which imples \e{1.Lp-divergence}.
\end{proof}






